Octuplet Loss: Make Face Recognition Robust to Image Resolution

Image resolution, or in general, image quality, plays an essential role in the performance of today's face recognition systems. To address this problem, we propose a novel combination of the popular triplet loss to improve robustness against image resolution via fine-tuning of existing face recognition models. With octuplet loss, we leverage the relationship between high-resolution images and their synthetically down-sampled variants jointly with their identity labels. Fine-tuning several state-of-the-art approaches with our method proves that we can significantly boost performance for cross-resolution (high-to-low resolution) face verification on various datasets without meaningfully exacerbating the performance on high-to-high resolution images. Our method applied on the FaceTransformer network achieves 95.12% face verification accuracy on the challenging XQLFW dataset while reaching 99.73% on the LFW database. Moreover, the low-to-low face verification accuracy benefits from our method. We release our code to allow seamless integration of the octuplet loss into existing frameworks.

==> tables/tab-tarfar.tex <==
% Table generated by Excel2LaTeX from sheet 'Tables'
\begin{tabular}{lccccccc}
\toprule
\multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{$r$ [px]} & \multicolumn{2}{c}{TAR@FAR=0.001} & \multicolumn{2}{c}{TAR@FAR=0.01} & \multicolumn{2}{c}{TAR@FAR=0.1} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}      &       & Baseline & $\lossOct$ & Baseline & $\lossOct$ & Baseline & $\lossOct$ \\
\midrule
\multirow{5}[2]{*}{LFW} & 7     & \cl 0.07 & 53,33 \smaller{ (\clg{+53,26})} & \cl 0.80 & 82,80 \smaller{ (\clg{+82,00})} & \cl 9.37 & 97,10 \smaller{ (\clg{+87,73})} \\
      & 14    & \cl 30.63 & 90,70 \smaller{ (\clg{+60,07})} & \cl 41.77 & 97,90 \smaller{ (\clg{+56,13})} & \cl 64.43 & 99,67 \smaller{ (\clg{+35,24})} \\
      & 28    & \cl 95.67 & 97,70 \smaller{ (\clg{+2,03})} & \cl 98.30 & 99,40 \smaller{ (\clg{+1,10})} & \cl 99.60 & 99,73 \smaller{ (\clg{+0,13})} \\
      & 56    & \cl 98.70 & 99,00 \smaller{ (\clg{+0,30})} & \cl 99.47 & 99,53 \smaller{ (\clg{+0,06})} & \cl 99.73 & 99,77 \smaller{ (\clg{+0,04})} \\
      & 112   & \cl 98.97 & 99,03 \smaller{ (\clg{+0,06})} & \cl 99.53 & 99,57 \smaller{ (\clg{+0,04})} & \cl 99.73 & 99,77 \smaller{ (\clg{+0,04})} \\
\midrule
XQLFW &       & \cl 0.03 & 69,50 \smaller{ (\clg{+69,47})} & \cl 0.27 & 83,10 \smaller{ (\clg{+82,83})} & \cl 57.40 & 95,07 \smaller{ (\clg{+37,67})} \\
\bottomrule
\end{tabular}%






% This is for separating the columns!
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}      &       & Baseline & $\lossOct$ & Baseline & $\lossOct$ & Baseline & $\lossOct$ \\
